Refining time-space traffic diagrams: A simple multiple linear regression model

A time-space traffic (TS) diagram, which presents traffic states in time-space cells with color, is an important traffic analysis and visualization tool. Despite its importance for transportation research and engineering, most TS diagrams that have already existed or are being produced are too coarse to exhibit detailed traffic dynamics due to the limitations of existing information technology and traffic infrastructure investment. To increase the resolution of a TS diagram and enable it to present ample traffic details, this paper introduces the TS diagram refinement problem and proposes a multiple linear regression-based model to solve the problem. Two tests, which attempt to increase the resolution of a TS diagram 4 and 16 times, are carried out to evaluate the performance of the proposed model. Data collected at different times, in different locations and even in different countries are employed to thoroughly evaluate the accuracy and transferability of the proposed model. Strict tests with diverse data show that the proposed model, despite its simplicity, is able to refine a TS diagram with promising accuracy and reliable transferability. The proposed refinement model will "save" widely existing TS diagrams from their blurry "faces" and enable TS diagrams to show more traffic details.

==> RefineTXPlot_R2 <==
% Generated by IEEEtran.bst, version: 1.13 (2008/09/30)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{Zheng2010}
Z.~Zheng, S.~Ahn, and C.~M. Monsere, ``{Impact of traffic oscillations on
  freeway crash occurrences},'' \emph{Accident Analysis and Prevention},
  vol.~42, no.~2, pp. 626--636, 2010.

\bibitem{Zheng2011b}
Z.~Zheng, S.~Ahn, D.~Chen, and J.~Laval, ``{Applications of wavelet transform
  for analysis of freeway traffic: Bottlenecks, transient traffic, and traffic
  oscillations},'' \emph{Transportation Research Part B}, vol.~45, no.~2, pp.
  372--384, 2011.

\bibitem{Lu2017}
L.~Lu, J.~Wang, Z.~He, and C.-y. Chan, ``{Real-time estimation of freeway
  travel time with recurrent congestion based on sparse detector data},'' 2017.

\bibitem{Grumert2018}
E.~F. Grumert, A.~Tapani, and X.~Ma, ``{Characteristics of variable speed limit
  systems},'' \emph{European Transport Research Review}, vol.~10, no.~21, 2018.

\bibitem{Chen2020}
X.~Chen, T.~Li, Z.~Ma, and J.~Sun, ``{Integrated mainline and ramp signal
  control for expressway on-ramp bottleneck with unequal lane-setting},''
  \emph{Journal of Intelligent Transportation Systems: Technology, Planning,
  and Operations}, vol.~26, no.~1, pp. 100--115, 2021.

\bibitem{Wang2022}
Y.~Wang, M.~Zhao, X.~Yu, Y.~Hu, P.~Zheng, W.~Hua, L.~Zhang, S.~Hu, and J.~Guo,
  ``{Real-time joint traffic state and model parameter estimation on freeways
  with fixed sensors and connected vehicles: State-of-the-art overview,
  methods, and case studies},'' \emph{Transportation Research Part C}, vol.
  134, no. October 2021, p. 103444, 2022.

\bibitem{Chen2004b}
C.~Chen, A.~Skabardonis, and P.~Varaiya, ``{Systematic Identification of
  Freeway Bottlenecks},'' \emph{Transportation Research Record: Journal of the
  Transportation Research Board}, vol. 1867, no.~1, pp. 46--52, 2004.

\bibitem{Ban2008}
X.~J. Ban, L.~Chu, and H.~Benouar, ``{Bottleneck Identiﬁcation and
  Calibration for Corridor Management Planning},'' \emph{Transportation
  Research Record: Journal of the Transportation Research Board}, vol. 1999,
  no.~5, pp. 40--53, 2008.

\bibitem{Wan2020}
Q.~Wan, G.~Peng, Z.~Li, and F.~H.~T. Inomata, ``{Spatiotemporal trajectory
  characteristic analysis for traffic state transition prediction near
  expressway merge bottleneck},'' \emph{Transportation Research Part C:
  Emerging Technologies}, vol. 117, no. February 2019, p. 102682, 2020.

\bibitem{He2015}
Z.~He, S.~He, and W.~Guan, ``{A figure-eight hysteresis pattern in macroscopic
  fundamental diagrams and its microscopic causes},'' \emph{Transportation
  Letters}, vol.~7, no.~3, pp. 133--142, 2015.

\bibitem{Dai2017}
X.~Ma, Z.~Dai, Z.~He, J.~Ma, Y.~Wang, and Y.~Wang, ``{Learning Traffic as
  Images: A Deep Convolution Neural Network for Large-scale Transportation
  Network Speed Prediction},'' \emph{Sensors}, vol.~17, no.~4, p. 818, 2017.

\bibitem{Zhang2017c}
Z.~Zhang, Y.~Wang, P.~Chen, Z.~He, and G.~Yu, ``{Probe data-driven travel time
  forecasting for urban expressways by matching similar spatiotemporal traffic
  patterns},'' \emph{Transportation Research Part C: Emerging Technologies},
  vol.~85, no. October, pp. 476--493, 2017.

\bibitem{He2020}
Z.~He, W.~Zhang, and N.~Jia, ``{Estimating Carbon Dioxide Emissions of Freeway
  Traffic: A Spatiotemporal Cell-Based Model},'' \emph{IEEE Transactions on
  Intelligent Transportation Systems}, vol.~21, no.~5, pp. 1976--1986, 2020.

\bibitem{He2019}
Z.~He, Y.~Lv, L.~Lu, and W.~Guan, ``{Constructing spatiotemporal speed contour
  diagrams: using rectangular or non-rectangular parallelogram cells?}''
  \emph{Transportmetrica B}, vol.~7, no.~1, pp. 44--60, 2019.

\bibitem{Treiber2002}
M.~Treiber and D.~Helbing, ``{Reconstructing the spatio-temporal traffic
  dynamics from stationary detector data},'' \emph{Cooper@tive Tr@nsport@},
  vol.~24, pp. 1--24, 2002.

\bibitem{Treiber2011a}
M.~Treiber, A.~Kesting, and R.~E. Wilson, ``{Reconstructing the Traffic State
  by Fusion of Heterogeneous Data},'' \emph{Computer-Aided Civil and
  Infrastructure Engineering}, vol.~26, no.~6, pp. 408--419, 2011.

\bibitem{Wang2005}
Y.~Wang and P.~Papageorgiou, ``{Real-time freeway traffic state estimation
  based on extended Kalman filter: a general approach},'' \emph{Transportation
  Research Part B: Methodological}, vol.~39, no.~2, pp. 141--167, feb 2005.

\bibitem{Wang2007}
Y.~Wang, M.~Papageorgiou, and A.~Messmer, ``{Real-Time Freeway Traffic State
  Estimation Based on Extended Kalman Filter: A Case Study},''
  \emph{Transportation Science}, vol.~41, no.~2, pp. 167--181, 2007.

\bibitem{Wang2008a}
Y.~Wang, M.~Papageorgiou, and A.~Messmer, ``{Real-time freeway traffic state estimation based on extended Kalman
  filter: Adaptive capabilities and real data testing},'' \emph{Transportation
  Research Part A: Policy and Practice}, vol.~42, no.~10, pp. 1340--1358, 2008.

\bibitem{Laval2012}
J.~Laval, Z.~He, and F.~Castrillon, ``{Stochastic extension of newell's
  three-detector method},'' \emph{Transportation Research Record}, vol. 2315,
  no. 2315, pp. 73--80, 2012.

\bibitem{Deng2013}
W.~Deng, H.~Lei, and X.~Zhou, ``{Traffic state estimation and uncertainty
  quantification based on heterogeneous data sources: A three detector
  approach},'' \emph{Transportation Research Part B: Methodological}, vol.~57,
  pp. 132--157, 2013.

\bibitem{He2017}
Z.~He, L.~Zheng, P.~Chen, and W.~Guan, ``{Mapping to Cells: A Simple Method to
  Extract Traffic Dynamics from Probe Vehicle Data},'' \emph{Computer-Aided
  Civil and Infrastructure Engineering}, vol.~32, no.~3, pp. 252--267, 2017.

\bibitem{He2017a}
Z.~He and Z.~Liang, ``{Visualizing traffic dynamics based on floating car
  data},'' \emph{Journal of Transportation Engineering}, vol. 143, no.~5, p.
  04017005, 2017.

\bibitem{Seo2017}
T.~Seo, A.~M. Bayen, T.~Kusakabe, and Y.~Asakura, ``{Traffic state estimation
  on highway: A comprehensive survey},'' \emph{Annual Reviews in Control},
  vol.~43, pp. 128--151, 2017.

\bibitem{Tsai1984}
R.~Tsai and T.~Huang, ``{Multi-Frame Image Restoration and Registration},''
  \emph{Advances in Computer Vision and Image Processing}, vol.~1, pp.
  317--339, 1984.

\bibitem{Irani1990}
M.~Irani and S.~Peleg, ``{Super resolution from image sequences},'' in
  \emph{Proceedings - International Conference on Pattern Recognition}, vol.~2,
  1990, pp. 115--120.

\bibitem{Wang2015}
Z.~Wang, D.~Liu, J.~Yang, W.~Han, and T.~Huang, ``{Deep networks for image
  super-resolution with sparse prior},'' in \emph{Proceedings of the IEEE
  International Conference on Computer Vision}, vol. 2015 Inter, 2015, pp.
  370--378.

\bibitem{Dong2016}
C.~Dong, C.~C. Loy, K.~He, and X.~Tang, ``{Image super-resolution using deep
  convolutional networks},'' \emph{IEEE Transactions on Pattern Analysis and
  Machine Intelligence}, vol.~38, no.~2, pp. 295--307, 2016.

\bibitem{Zhang2018}
Y.~Zhang, Y.~Tian, Y.~Kong, B.~Zhong, and Y.~Fu, ``{Residual Dense Network for
  Image Super-Resolution},'' in \emph{Proceedings of the IEEE Computer Society
  Conference on Computer Vision and Pattern Recognition}, 2018, pp. 2472--2481.

\bibitem{Wu2021}
Y.~Wu, B.~Teufel, L.~Sushama, S.~Belair, and L.~Sun, ``{Deep Learning-Based
  Super-Resolution Climate Simulator-Emulator Framework for Urban Heat
  Studies},'' \emph{Geophysical Research Letters}, vol.~48, no.~19, pp. 1--11,
  2021.

\bibitem{Zhang2022}
K.~Zhang, X.~Feng, N.~Jia, L.~Zhao, and Z.~He, ``{TSR-GAN: Generative
  Adversarial Networks for Traffic State Reconstruction with Time Space
  Diagrams},'' \emph{Physica A: Statistical Mechanics and its Applications},
  vol. 591, p. 126788, 2022.

\bibitem{HanshinExp2018}
{Hanshin Exp. Co. Ltd.}, ``{Zen Traffic Data},''
  \emph{https://zen-traffic-data.net/english/}, 2018.

\bibitem{Dahiyal2020}
G.~Dahiyal, Y.~Asakura, and W.~Nakanishi, ``{A study of speed-density
  functional relations for varying spatiotemporal resolution using Zen Traffic
  Data},'' in \emph{23rd IEEE International Conference on Intelligent
  Transportation Systems (ITSC)}, 2020.

\bibitem{NGSIM2006}
{U.S. Federal Highway Administration}, ``{The Next Generation Simulation
  Program (NGSIM)},''
  \emph{http://ops.fhwa.dot.gov/trafficanalysistools/ngsim.htm}, 2006.

\bibitem{Zielke2008}
B.~Zielke, R.~Bertini, and M.~Treiber, ``{Empirical Measurement of Freeway
  Oscillation Characteristics: An International Comparison},''
  \emph{Transportation Research Record: Journal of the Transportation Research
  Board}, vol. 2088, pp. 57--67, 2008.

\bibitem{Laval2010}
J.~Laval and L.~Leclercq, ``{A mechanism to describe the formation and
  propagation of stop-and-go waves in congested freeway traffic.}''
  \emph{Philosophical transactions. Series A, Mathematical, physical, and
  engineering sciences}, vol. 368, no. 1928, pp. 4519--41, oct 2010.

\bibitem{Chen2012i}
D.~Chen, J.~Laval, S.~Ahn, and Z.~Zheng, ``{Microscopic traffic hysteresis in
  traffic oscillations: A behavioral perspective},'' \emph{Transportation
  Research Part B: Methodological}, vol.~46, no.~10, pp. 1440--1453, dec 2012.

\bibitem{Jiang2014}
R.~Jiang, M.-B. Hu, H.~M. Zhang, Z.-Y. Gao, B.~Jia, Q.-S. Wu, B.~Wang, and
  M.~Yang, ``{Traffic experiment reveals the nature of car-following.}''
  \emph{PloS one}, vol.~9, no.~4, p. e94351, jan 2014.

\bibitem{He2015a}
Z.~He, L.~Zheng, and W.~Guan, ``{A simple nonparametric car-following model
  driven by field data},'' \emph{Transportation Research Part B:
  Methodological}, vol.~80, no. 2015, pp. 185--201, 2015.

\bibitem{Treiber}
M.~Treiber and A.~Kesting, \emph{{Traffic flow dynamics: Data, models and
  simulation}}.\hskip 1em plus 0.5em minus 0.4em\relax Springer, 2013.

\bibitem{Laval2014}
J.~A. Laval, C.~S. Toth, and Y.~Zhou, ``{A parsimonious model for the formation
  of oscillations in car-following models},'' \emph{Transportation Research
  Part B: Methodological}, vol.~70, pp. 228--238, dec 2014.

\bibitem{Li2020a}
L.~Li, R.~Jiang, Z.~He, X.~M. Chen, and X.~Zhou, ``{Trajectory data-based
  traffic flow studies: A revisit},'' pp. 225--240, 2020.

\bibitem{Newell1982}
G.~F. Newell, \emph{{Applications of Queueing Theory}}, 1982.

\bibitem{Cassidy1995}
M.~J. Cassidy and J.~R. Windover, ``{Methodology for assessing the dynamics of
  freeway traffic flow},'' pp. 73--79, 1995.

\bibitem{Chiabaut2009}
N.~Chiabaut, C.~Buisson, and L.~Leclercq, ``{Fundamental diagram estimation
  through passing rate measurements in congestion},'' \emph{IEEE Transactions
  on Intelligent Transportation Systems}, vol.~10, no.~2, pp. 355--359, 2009.

\bibitem{He2017c}
Z.~He, L.~Zheng, L.~Song, and N.~Zhu, ``{A Jam-Absorption Driving Strategy for
  Mitigating Traffic Oscillations},'' \emph{IEEE Transactions on Intelligent
  Transportation Systems}, vol.~18, no.~4, pp. 802--813, 2017.

\end{thebibliography}

